Misinfo Reaction Frames: Reasoning about Readers' Reactions to News Headlines

Even to a simple and short news headline, readers react in a multitude of ways: cognitively (e.g. inferring the writer's intent), emotionally (e.g. feeling distrust), and behaviorally (e.g. sharing the news with their friends). Such reactions are instantaneous and yet complex, as they rely on factors that go beyond interpreting factual content of news. We propose Misinfo Reaction Frames (MRF), a pragmatic formalism for modeling how readers might react to a news headline. In contrast to categorical schema, our free-text dimensions provide a more nuanced way of understanding intent beyond being benign or malicious. We also introduce a Misinfo Reaction Frames corpus, a crowdsourced dataset of reactions to over 25k news headlines focusing on global crises: the Covid-19 pandemic, climate change, and cancer. Empirical results confirm that it is indeed possible for neural models to predict the prominent patterns of readers' reactions to previously unseen news headlines. Additionally, our user study shows that displaying machine-generated MRF implications alongside news headlines to readers can increase their trust in real news while decreasing their trust in misinformation. Our work demonstrates the feasibility and importance of pragmatic inferences on news headlines to help enhance AI-guided misinformation detection and mitigation.

==> moved_from_intro.tex <==
%However, effectiveness is dependent on generation quality (\S\ref{sec:gen}), urging caution for deployment of misinformation countering systems. 

%\ms{I would add a paragraph introducing the corpus and that we train models to predict MBF from headlines. You can frame it as a case study of two/three subjects of misinformation? And potentially explain why you're focusing on specific topics instead of a "general" framework?
%Briefly, you can mention the main results of how well models can generate MBFs from new headlines }

%\ms{Say something like ``To showcase the usefulness of this paradigm, we investigate how much MBF explanations help with increaes/decrease trust in headlines, and how it helps detect misinfo. Describe the key results, copy-pasting from what you wrote below.}

%We apply these pragmatic frame annotations to three paradigms within the study of misinformation where interpreting intent and reader perception is key: 

%\ms{You could re-iterate some of these points in a contributions paragraph? And move the related-work-y stuff to section 2, where you could have a (sub)section discussing the need for MBF as a new view on misinfo (and contrasting to previous work)...}
%\paragraph{\underline{Misinformation Detection}}

%As shown by prior work \cite{Resnick2021InformedCC}, crowdsource workers from user studies can accurately identify instances of misinformation. We show that our pragmatic frames can be used to improve performance of misinformation detection models [add results, best performance (84\% F1)]. However, this is a challenging task, and we highlight failures of current misinformation detection models (See \S\ref{sec:error_analysis}) to aid in future research. 

%\paragraph{\underline{Understanding Reader Behavior}}

%Likelihood of user spread ratings obtained from user studies also correlates with actual reader behavior on social media \cite{Mosleh2020SelfreportedWT}. Importantly, our pragmatic frames incorporate variation in personal interpretation of the meaning behind news media %the \ms{that's not true tho, we don't ask people what their prior attitudes about the topic was, right?}implicit role that personal belief systems play in interpretation 
%\cite{Hall1973EncodingAD} and social commonsense implications \cite{mindreaders,Sap2019ATOMICAA} of headlines, going beyond purely rhetorical techniques or stylometry \cite{mihalcea-strapparava-2009-lie,rashkin-etal-2017-truth,karimi-etal-2018-multi, zellers2019neuralfakenews}. 
%\paragraph{\underline{Countering Misinformation}}
%Finally, we show that the MBF corpus can be used to obtain machine-generated explanations of news headlines.  Notably, our results show that machine-generated MBF inferences affect readers' trust in headlines and for the best model there is a statistically significant correlation (Pearson's $r$=0.24, $p$=0.018) with labels of trustworthiness. However, effectiveness is dependent on generation quality (\S\ref{sec:gen}), urging caution for deployment of misinformation countering systems. 
%\ms{need to discuss the classification of true vs fake news too:}
% We can also learn more about the perceived reliability of the news or overall appeal of the article given the likelihood the reader would share it within their network.
%\ms{Possibly, move this to \S 2}
% Misinfo Belief Frames go beyond linguistic meaning and focus on the way in which readers' prior beliefs project meaning onto news headlines, inspired by frame semantics \cite{Fillmore1976FRAMESA}.
% We also introduce the \textbf{MBF corpus} consisting of 66.7k inferences over 24.3k headlines.
%Our formalism captures how readers view the implications of news events through the lens of pragmatic frames.
%Inspired by frame semantics \cite{Fillmore1976FRAMESA}, %\yejin{actually, when referring to fillmore76, the more accurate term is ''frame semantics'' not the other way...} 
% we provide a means of situating news content within a broader context. Misinfo Belief Frames go beyond linguistic meaning and focus on the way in which readers' prior beliefs project meaning onto news headlines.
 %\yejin{it reads weird that stylometry is one of the key components of our frames... is it necessary there?} 

%The rapid dissemination of information online has led to an increasing problem of falsified or misleading news spread on discussion forums like Twitter, Reddit and Facebook \cite{Vosoughi1146,10.1145/3313831.3376784}. This misinformation can reinforce sociopolitical divisions \cite{Vidgen2020DetectingEA,voterfraud}, pose risks to public health \cite{10.1145/3274327}, and undermine efforts to educate the public about global crises \cite{climate}.
%\ec{not sure how much "Misinformation Belief Graphs Framework" at the top of figure helps}
%\begin{center} Distinguishing misinformation from real news often requires \textit{extrinsic}\footnote{By \textit{intrinsic} and \textit{extrinsic} knowledge, we respectively refer to knowledge that is or is not explicitly given in the context of a news article/headline.}  knowledge pertaining to claims, including commonsense knowledge. \end{center}
% Prior work has shown the effectiveness of lexical techniques and large-scale language modeling for misinformation detection \cite{mihalcea-strapparava-2009-lie,rashkin-etal-2017-truth,karimi-etal-2018-multi, zellers2019neuralfakenews}. However, stylometry alone cannot reliably measure trustworthiness of news \cite{schuster2020limitations}. Reliable sources can use similar persuasive techniques and linguistic cues to misinformation. Prior binary labeling schemes also hide the impact and subliminal messaging captured by misinformation. 
%news outlet sources restricts our ability to detect misinformation when it comes from sources with variable reliability, previously unknown sources, and articles taken out of a source-based context. Relying on linguistic cues like lexical sentiment also narrows the scope of misinformation that can be captured by current misinformation detection systems. While \cite{da-san-martino-etal-2019-fine} uses explicit propagandistic rhetorical techniques such as ``name-calling" \cite{name-calling} as indicators for propaganda detection and \cite{perez-rosas-etal-2018-automatic} uses pyscholinguistic features for detecting biased, falsified or misleading news, many instances of misinformation related to health and climate news contain factually incorrect information presented without obvious inflammatory or exaggerated language (e.g. the fake news headline \textit{``Wearing a mask causes hypoxia, hypercapnia, and pneumonia."}). Concurrently, using rhetorical techniques alone for determining misinformation leads to some real news headlines being labeled as misinformation due to sensationalized language designed to increase click-through rates of news articles or lack of disambiguation between the context of the article and context provided by quotations (e.g. the real news headline \textit{``No-deal Brexit threatens `innumerable problems' for environmental projects'"}\footnote{Propaganda detection models from \cite{da-san-martino-etal-2019-fine} predict that this headline contains an instance of the ``exaggeration" propaganda technique \cite{exaggeration}.}).  
%:
%\begin{itemize}
%\item Writer's Intention. What is being implied by the original writer of the headline about mentioned entities or the topic? 
%\item Reader's Perception. How would the reader perceive the headline (e.g. emotional reactions that are likely to be invoked)?
%\item Reader's Action. What action is it mostly likely that the reader would take as a consequence of reading the headline?
%\item Likelihood of Spread. What is the likelihood that the headline would lead to readers sharing the article?
%\end{itemize}

%These implications construct a commonsense rationale designed for increased understanding of \textit{intentions} behind a real and falsified news events. These rationales are directly conveyed by the content of event and help to further machine reading comprehension of misinformation. 

%\ms{Not sure I love ``case study'' but I wrote it anyways}
%As a case study, we introduce the \textbf{MBF corpus} to study the implications of misinformation related to two global crises: the Covid-19 pandemic and climate change.
%Using our pragmatic frames, we collect 66.7k annotations for 24.3k news headlines from trustworthy and untrustworthy sources.
% Covering 66.7k MBF inferences over 24.3k news headlines, we use our corpus to train neural models to make inferences about unseen headlines.
%With this corpus, we investigate neural models' ability to generate MBF for previously unseen headlines, and whether model-generated inferences can influence readers' trust in misinformation.

%\ms{Please edit this paragraph}

%We use the pragmatic frames represented by MBF corpus inferences to analyze differences between misinformation and real news in the climate and Covid health domains.
%Our results show that surface-level linguistic patterns are not enough for detecting misinformation, as zero-shot performance of stylometric models on our dataset is substantially lower (37\% F1) than models trained on MBF. 
% We also compare against prior formalisms for identifying rhetorical techniques in descriptions of news events using zero-shot prediction to show that emerging misinformation requires new understandings of how bad actors convey malicious intentions (rhetoric detection models achieve a validation F1 score of 45.20\% at misinformation detection compared to a F1 score of 90.35\% for task-specific models). 
% Finally, we contribute MBF benchmark results from large-scale models and show domain-specific pre-training improves misinformation detection over MBF headlines by 4.77\%. % to generate MARS inferences on unseen headlines.\ec{i cannot parse this sentence..} 
 %\fr{Affect them in desired directions? :)}

%\begin{center} Binary classification hides the fact not all misinformation is created equal - there are varying risks to society posed by misinformation. \end{center}
